Single-Leg Revenue Management with Advice

Single-leg revenue management is a foundational problem of revenue management that has been particularly impactful in the airline and hotel industry: Given $n$ units of a resource, e.g. flight seats, and a stream of sequentially-arriving customers segmented by fares, what is the optimal online policy for allocating the resource. Previous work focused on designing algorithms when forecasts are available, which are not robust to inaccuracies in the forecast, or online algorithms with worst-case performance guarantees, which can be too conservative in practice. In this work, we look at the single-leg revenue management problem through the lens of the algorithms-with-advice framework, which attempts to harness the increasing prediction accuracy of machine learning methods by optimally incorporating advice about the future into online algorithms. In particular, we characterize the Pareto frontier that captures the tradeoff between consistency (performance when advice is accurate) and competitiveness (performance when advice is inaccurate) for every advice. Moreover, we provide an online algorithm that always achieves performance on this Pareto frontier. We also study the class of protection level policies, which is the most widely-deployed technique for single-leg revenue management: we provide an algorithm to incorporate advice into protection levels that optimally trades off consistency and competitiveness. Moreover, we empirically evaluate the performance of these algorithms on synthetic data. We find that our algorithm for protection level policies performs remarkably well on most instances, even if it is not guaranteed to be on the Pareto frontier in theory. Our results extend to other unit-cost online allocations problems such as the display advertising and the multiple secretary problem together with more general variable-cost problems such as the online knapsack problem.

==> CR_bounds.tex <==
\section{Bounds on the Competitive Ratio}

Notation: $G(y) = E[Y \mathds{1}(Y \geq F^{-1}(1-y))]$.

Assumption: $G(1) = 1$

Observe that $Opt(i) = i G\left(\min\{B/i, 1\}\right)$.

\begin{theorem}
	The competitive ratio can be characterized as follows:
	\begin{align*}
		CR(G,T) = \sup_{Alg} \inf_{t\in [T]} \frac{Opt(t)}{Alg(t)} = \inf\left\{c\ \biggr\lvert\ G^{-1}\left(\frac{Opt(1)}{c}\right) + \sum_{i=1}^T G^{-1}\left( \frac{1}{c} \cdot \{Opt(i+1) - Opt(i)\} \right) \leq B  \right\}
	\end{align*}	
\end{theorem}

\begin{proof}
	This is a special case of a latter theorem. 
\end{proof} 

\subsection{Lower Bounds}

Set $G(x) = x^r$ for $r \in (0,1]$. Then, by the above theorem, the competitive ratio $c$ satisfies
\begin{align*}
	\frac{1}{c^{1/r}} &\left[ 1 + \sum_{i=1}^T \{(i+1)^{1-r} - i^{1-r}\}^{1/r} \right] \leq 1\\
	\implies c &\geq \left[ 1 + \sum_{i=1}^T \{(i+1)^{1-r} - i^{1-r}\}^{1/r} \right]^r\\
	&\geq \left[ 1 + \sum_{i=1}^T \{(i+1)^{1-r} - i^{1-r}\}^{1/r} \frac{\{(i+1)^{r} + i^{r}\}^{1/r}}{\{(i+1)^{r} + i^{r}\}^{1/r}} \right]^r\\
	&\geq \left[1 + \sum_{i=1}^T \frac{\{1 - [(i+1)^{r} i^{1-r} - (i+1)^{1-r} i^{r}]\}^{1/r}}{2^{1/r} (i+1)} \right]^r\\
\end{align*}

Note that
\begin{align*}
	(i+1)^{r} i^{1-r} - (i+1)^{1-r} i^{r} &\leq r(i+1) + (1 -r)i - (i+1)^{1-r}i^r\\
	&\leq  r + i - i^{1-r}i^r\\
	&= r 
\end{align*}

Therefore,
\begin{align*}
	c &\geq \left[1 + \sum_{i=1}^T \frac{(1 - r)^{1/r}}{2^{1/r} (i+1)} \right]^r\\
	&\geq \frac{1-r}{2} \left[\sum_{i=1}^T \frac{1}{i+1} \right]^r\\	
	&\geq \frac{1-r}{2} \cdot \left\{\ln\left(\frac{T}{2}\right)\right\}^r
\end{align*}

The RHS is maximized at $r = 1 - (1/\ln\ln(T/2))$, which yields
\begin{align*}
	c \geq \frac{1}{\ln\ln(T/2)} \cdot \ln\left(\frac{T}{2}\right)^{1 - \frac{1}{\ln\ln(T/2)}} = \frac{\ln(T/2)}{e\cdot \ln\ln(T/2)}
\end{align*}



\subsection{Upper Bounds}


Fix $B = 1$. Set $x_i = \left(1 - \frac{Opt(i-1)}{Opt(i)}\right)/\Delta$, where $\Delta = \sum_{i=1}^T \left(1 - \frac{Opt(i-1)}{Opt(i)}\right)$. We will show that, this achieves a competitive ratio of a $\Delta$. To do so, we will use induction on $t \in [T]$. For the base case, it is straightforward to see that $Alg(1) = G(1/\Delta) \geq G(1)/\Delta = Opt(1)/\Delta$ because $G$ is non-decreasing and concave. Assume that $Alg(t) \geq Opt(t)/\Delta$ for some $t \in [T-1]$. Then,
\begin{align*}
	Alg(t+1) &= Alg(t) + G(x_i)\\
	&\geq Opt(t)/\Delta + G\left(\left(1 - \frac{Opt(t)}{Opt(t+1)}\right)/\Delta\right)  	
\end{align*}

First, observe that
\begin{align*}
	1 - \frac{Opt(t)}{Opt(t+1)} = 1 - \frac{t \cdot G(t)}{(t+1) \cdot G(t+1)} \leq 1 - \frac{t}{t+1} = \frac{1}{t+1}  
\end{align*}

Therefore, $G(x_i)/x_i \geq G(1/(T+1))/(1/(T+1)) = Opt(T+1)$ because $G$ is non-decreasing and concave. Hence, 
\begin{align*}
	Alg(t+1) &\geq Opt(t)/\Delta + G\left(\left(1 - \frac{Opt(t)}{Opt(t+1)}\right)/\Delta\right)\\
	&\geq Opt(t)/\Delta + \left(1 - \frac{Opt(t)}{Opt(t+1)}\right)\cdot \frac{1}{\Delta} \cdot Opt(t+1)\\
	&= Opt(t+1)/\Delta 	
\end{align*}

Finally, observe that $(1 - x) \leq \ln(1/x)$ for $x \in (0,1)$. Therefore, $\Delta \leq \ln(Opt(T)/Opt(1)) \leq \ln(\frac{TG(1/T)}{G(1)}) \leq \ln(T)$.

To do: Lower bounds and budgets
      








==> adverserial.tex <==
\section{Adverserial Setting with Known Distribution}

We will consider the online knapsack problem where the number of time steps is not known. Let $F$ be a reward distribution, which we will assume is known to the decision maker. Moreover, assume that we have a total capacity of $B$ and each item, if accepted with probability $x$, takes up $x$ units of this capacity (fluid model). At each time step, one item with reward from $F$ if offered. The total number of such time periods is not known and is non-adaptively selected by an adversary. 

%\subsection{Bad Example}
%
%Let $F$ be the uniform distribution on $[0,1]$ and set $B = 1$. Suppose the adversary picks the number of time periods to be 1 with probability $p$ and $T$ with probability $1-p$. First, note that if we pick an item with probability $x$, then the reward it yields is at most $E[Y \mathds{1}( Y > 1- x)] = x - x^2/2$. Therefore, for a decision maker that sets $x$ as the acceptance probability for the first time period and $(1/2 - x)/(T-1)$ for the rest of the periods, gets a reward equal to
%\begin{align*}
%	a(x,p) &\coloneqq p \cdot \left(x - \frac{x^2}{2}\right) + (1 - p) \left[ x - \frac{x^2}{2} + (T-1) \left( \frac{1 - x}{T-1} - \frac{(1 - x)^2}{2 ( T-1)^2}\right) \right]\\
%	&= x - \frac{x^2}{2} + (1 - p)\left(1 - x\right) - (1 - p)\frac{1 + x^2 -2x}{2(T-1)}\\
%	&= \frac{(1 - p)(2T - 3) + (2pT - 4p + 2)x - (T - p)x^2}{2(T-1)}
%\end{align*}
%
%Therefore, maximizing over $x$, we get
%\begin{align*}
%	Alg(p) = \max_x a(x,p) = \frac{(1-p)(2T - 3)(T - p) + (pT - 2p + 1)^2}{2(T-1)(T- p)}	
%\end{align*}
%
%On the other hand, if we knew the number of time periods, then the best possible expected reward is given by
%\begin{align*}
%	Opt(p) = p \cdot \frac{1}{2} + (1 - p) T \left( \frac{1}{T} - \frac{1}{2T^2} \right)
%\end{align*}
%
%For the worst case example, we would like to maximize the following ratio
%\begin{align*}
%	CR(p) = \frac{Opt(p)}{Alg(p)}
%\end{align*}
%
%Maximized it on Mathematica and got a constant.





==> advice.tex <==
\section{ML Advice}

\begin{theorem}
	$\gamma$-competitiveness and $\beta$-consistency are achievable if and only if the following water-filling algorithm spends less than the budget: At step $t$, fill enough water on the slots $1 \leq i \leq t$ to achieve the required fraction of $Opt(t)$. 
\end{theorem}

\begin{proof}
	The if part is trivial. For the only if part, suppose there is some allocation $(x_1, \dots, x_n)$ which achieves $\gamma$-competitiveness and $\beta$-consistency. Suppose there are water containers at each time step $i$ with capacity $x_i$. With each time step $t \in [T]$, we will associate a part of the allocation as follows: At each time step $t$, fill enough water into the containers at $1 \leq i \leq t$ to achieve the required competitive ratio. We will show via induction that, at the end of time step $t$, for each $1 \leq i \leq t$, one of the following conditions holds:
	\begin{itemize}
		\item the container at $i$ is at capacity
		\item the container is filled higher than our water-filling algorithm till time step $t$	
	\end{itemize}
 	For the base case $t=1$, note that our water-filling algorithm and the above procedure fill the same amount of water in the first container. Suppose the state is true after time t-1. First, observe that the higher up the water, the less reward we get for it. This observation in combination with the induction hypothesis implies that induction statement continues to hold after step $t$.
\end{proof}

To do: simple policy that splits budget, LP for advice


\section{Revenue Management}

We begin by formulating the problem of robust revenue management as an LP. First, we do so for the case of $k=1$, i.e., there is exactly one seat on the plane. Let $r_1 < r_2 < r_3 \dots < r_n$ be the possible fare classes.
\begin{align*}
	\max \quad &z\\
	 \text{s.t. }& z \leq \frac{\sum_{j=1}^i r_j x_j}{r_i} \quad \forall i \in [n]\\
	 &\sum_{i=1}^n x_i = 1\\
	 & x_j \geq 0 \quad \forall j \in [n]
\end{align*}

In the above LP, the variable $x_j$ denotes the probability with which we pick $r_j$ as our fare threshold, i.e.,  we accept every fare greater than or equal to $r_j$ with probability $x_j$. The LP is designed to maximize the competitive ratio against LBH (low-before-high) fare sequences of the type $r_1, \dots, r_i$. The following lemma establishes that the above LP yields the optimal competitive ratio.

\begin{lemma}
	The value of the LP equals the optimal competitive ratio. Moreover, the threshold-based online policy which sets the threshold to be $r_i$ with probability $x_i^*$, where $x^*$ is an optimal solution of the LP, is optimal. 	
\end{lemma}

\begin{proof}
	First, we will show that the LP-based policy yields a competitive ratio greater than or equal to the value of the LP, which we denote by $c$. By definition of the LP, the LP-based policy achieves a competitive ratio of $c$ against low-before-high fare sequences. Next, let us consider an arbitrary sequence of fares $r_{i_1}, \dots, r_{i_T}$. As the offline optimal always picks the highest fare, it does not depend on the order in which the fares arrive. Therefore, the offline optimal is the same for the sequence $r_{i_1}, \dots, r_{i_T}$ and $r_1, \dots, r_k$, where $k = \argmax_t r_{i_t}$. Furthermore, the LP-based algorithm performs worse on the latter. Hence, the competitive ratio is at least $c$ against all possible fare sequences.
	
	To prove optimality of the LP-based policy, consider any online policy. Let $x_i$ be the probability with which it accepts $r_i$ when presented with the complete increasing sequence $r_1, \dots, r_n$, and $z$ be its competitive ratio. Since online policies are non-anticipating, we get that $(z,x)$ forms a feasible solution to the LP. Therefore, $z \leq c$. Hence, we have shown that no online policy has a competitive ratio strictly greater than $c$.
\end{proof}

Suppose the ML advice is $(p_1, \dots, p_n)$, where $p_i$ denotes the probability with which $r_i$ will be the highest fare class to arrive. Then, we can modify the above LP to find the best competitiveness achievable for a particular level of consistency:
\begin{align*}
	\max \quad &z\\
	 \text{s.t. }& z \leq \frac{\sum_{j=1}^i r_j x_j}{r_i} \quad \forall i \in [n]\\
	 & \beta \leq \sum_{i=1}^n p_i \frac{\sum_{j=1}^i r_j x_j}{r_i}\\
	 &\sum_{i=1}^n x_i = 1\\
	 & x_j \geq 0 \quad \forall j \in [n]
\end{align*}


\subsection{General Case (Not complete)}

We will now relax the assumption that $k = 1$. For this general case, the crux of the argument lies in showing that, for random threshold based policies, the worst case instances are the ones in which $k$ copies of the fares appear in increasing order. We will refer to these as LBH instances. Fix threshold probabilities $x$ and the competitive ratio $c$. We would like to show that $c Opt(I) - Alg(x,I)$ is maximized at some LBH instance. For contradiction, suppose not. Let $I$ be the instance with maximum number of customers among the instances which maximize $c Opt(I) - Alg(x,I)$. First note that sorting the customers in increasing order of fares can only increase $c Opt(I) - Alg(x,I)$. Hence, we can assume that $I$ has customers sorted by fare. Let $r_i$ be the highest fare in $I$ and $r_j$ be the lowest fare included in $Opt(I)$. Moreover, since adding more customers with fares less than or equal to $r_j$ can also only decrease $c Opt(I) - Alg(x,I)$, we can assume that there are $k$ customers of every fare less than or equal to $r_j$ in $I$. Suppose there are less than $k$ customers with fare $r_i$. Then, by our assumption of maximality on $I$, adding another customer with fare $r_i$ to $I$ strictly decreases $c Opt(I) - Alg(x,I)$. Therefore, reducing one customer with fare $r_i$ strictly increases $c Opt(I) - Alg(x,I)$, which is a contradiction. Hence, there are $k$ customers with fare $r_i$ in $I$. Finally, increasing the number of customers with fares less than or equal to $r_i$ to $k$ can only decrease $c Opt(I) - Alg(x,I)$, thereby completing the proof.   


%\subsection{Protection Level Policy for the General Case (Working on this)}
%
%In this section, we define an LP to find a protection level policy which incorporates advice for a general $k$. This generalizes the treatment of Ball and Queyranne so we will use their notation. Let $f_1 > f_2 \dots > f_m$ be the fares and the number the available seats to denoted by $n$. Like Ball and Queyranne, we consider the continuous case, i.e., fraction customers can be selected. The following LP attempts to maximize the consistency while maintaining $\gamma$-competitiveness. Suppose the advice is that there will be $a_i$ customers of the fare type $f_i$ and let $Opt(a)$ be the optimal action when the advice is true.
%\begin{align*}
%	\max \quad & \\
%	 \text{s.t. }& \gamma f_{i'}n \leq \sum_{i=i'}^m f_i(Q_i - Q_{i+1}) \quad \forall i' \in [m]\\
%	 & \beta\cdot Opt(a) \leq \sum_{i=1}^n f_i y_i\\
%	 &\sum_{i=i'}^m y_i \leq Q_{i'} \quad \forall i' \in [m]\\
%	 & y_i \leq a_i \quad \forall i \in [m]\\
%	 & Q_i \geq Q_{i+1},\ 0 \leq Q_i \leq n \quad \forall i \in [m]\\
%	 & y_i \geq 0 \quad \forall i \in [m]
%\end{align*}








==> optimal_policy.tex <==
\section{Optimal Policy}

Let $T$ be the upper bound on the possible number of items that will be offered by the adversary and $F$ be the distribution of rewards. We will assume that $F$ is discrete with support $\{r_1, \dots, r_K\}$, and is known to the decision-maker. Then, the competitive ratio is given by the value of the zero-sum game between the decision-maker and the adversary which can be described as follows:
\begin{itemize}
	\item The strategy of the adversary is the number of items to offer $t \in \{1, \dots, T\}$.
	\item The strategy set of the decision-maker is a description of the budget allocation $\{x \in \R_{\geq 0}^T \mid \sum_{i} x_i = B\}$
	\item The payoff to the decision-maker from strategy profile $(x,t)$ is given by the competitive ratio for $t$ items, i.e.,
		\begin{align*}
			u(x,t) = \frac{\sum_{i= 1}^t E[Y \mathds{1}(X \geq F^{-1}(1 - x_i))]}{Opt(t)}	
		\end{align*}
		where $Opt(t)$ is the optimal reward when the number of items to be offered is known
\end{itemize}

Observe that $x \mapsto E[Y \mathds{1}(Y \geq F^{-1}(1 - x))]$ is simply the area between the graph of $F$ and the Y axis between the points $1$ and $1 - x$, thereby making the function piece-wise linear concave function. This makes the game a convex game.

We can write an LP to compute the optimal policy when $F(\{r_j\}) =q_j$:
\begin{align*}
	\max \quad &z\\
	 \text{s.t. }& z \leq \frac{\sum_{i=1}^t \sum_{j=1}^K y_{ij} r_j}{Opt(t)} \quad \forall t \in [T]\\
	 & 0 \leq y_{ij} \leq q_j \quad \forall j \in [K], i \in [T]\\
	 &\sum_{i=1}^T x_i = B\\
	 & x_i \geq 0 \quad \forall i \in [T]
\end{align*}


 

==> revenue_management.tex <==
\section{TODO}

\begin{itemize}
	\item Algorithm performs better than simple policy
	\item Economic aspects of the pareto-frontier	
\end{itemize}


Next, we define two classes of online algorithms that will play a central role in our results: protection-level-policy based online algorithms and threshold-based algorithms.

\subsection{Protection-level-policy-based Online Algorithms}

Protection level policies are the method-of-choice for single-leg revenue management in the airline industry, and have garnered extensive attention in the revenue management literature~\citep{talluri2004theory, ball2009toward}. It is a form of quantity control parameterized by protection levels $0 \leq Q_1 \leq Q_{2} \leq \dots \leq Q_m = n$: the firm accepts at most $Q_i$ customers with fares $f_i$ or lower. The idea stems from the need to preserve capacity for higher paying customers that might arrive in the future. More precisely, on an instance $s_1, \dots s_T$ where $s_t = f_j$ for some $j \in [m]$, the fraction of $s_t$ accepted by the protection level policy with protection levels $Q = (Q_1, \dots, Q_m)$ can be iteratively defined as
\begin{align*}
	x_t = \max\left\{ x \in [0,1]\ \biggr\lvert\ x + \sum_{i=1}^{t-1} x_i\mathds{1}(s_i \leq f_k) \leq Q_k \text{ for all } k \leq j \right\}
\end{align*}

To incorporate advice, we consider meta online-algorithms that first map the advice $D \in \Delta(\A)$ to a vector of protection levels $Q(D)$, and then run the protection level policy with protection levels $Q(D)$ on the input instance. Different maps result in different protection-level-based online algorithms that incorporate advice.

%\subsection{Threshold-based Online Algorithms}
% 
%Threshold-based online algorithms use the advice to probabilistically select a threshold fare and then select all customers with fare greater than or equal to the threshold, i.e., a threshold based algorithm maps each advice $D \in \Delta(\A)$ to a point $x(D)$ in the $m-1$ dimensional probability simplex $\Delta^{m-1} \coloneqq \{x \in \R_+^m \mid \|x\|_1 = 1\}$, picks the fare $f_i$ to be the threshold with probability $x_i$, and accepts every customer with fare greater than or equal to threshold fare in the input instance while capacity remains.



\section{Revenue Management}

In this section, we consider the problem of single leg revenue management as defined in \citet{ball2009toward}. For completeness, we restate the problem here. Suppose an airline wants to sell tickets for a direct flight that has a capacity of $n$. Moreover, assume that the customers can belong to one of $m$ fare classes $f_1 > f_2 > \dots f_m$ which determines the amount they are willing to pay for a seat on the flight. \citet{ball2009toward} study the online problem where the customers arrive sequentially and the airline has to make an irrevocable decision to either accept or reject each customer. If accepted, the airline receives a revenue equal to the fare class of the customer. The goal is to find an algorithm to maximize the worst-case competitive ratio, i.e., the ratio of the performance of the online algorithm to that of the offline optimal when the instance is chosen adversarially. Like \citet{ball2009toward} do for the $m > 2$ fare-class case, we will work in the continuous demand setting where customers can be accepted partially. \citet{ball2009toward} describe two policies that achieve the optimal competitive ratio of $\Delta = \sum_{i=1}^m \left( 1 - \frac{f_{i+1}}{f_{i}}\right)$, where we set $f_{m+1} = 0$. Refer to the section on Multiple-Fare Classes of \citet{ball2009toward} for more details.

\begin{definition}
	An instance $I$ of the robust revenue management problem consists of a finite sequence of fares from the set $F = \{f_1, f_2, \dots, f_m\}$.
\end{definition}

\begin{definition}
	An advice is a vector $A \in \R_+^m$, where $A_i$ specifies how many customers with fare type $f_i$ are predicted to arrive.	We will abuse notation and also use $A$ to denote the instance in which $A_i$ customers with fare $f_i$ arrive in increasing order of fares.
\end{definition}

\begin{definition}
	On an instance $I$, $Opt(I)$ represents the revenue generated by the highest $n$ fares, i.e. the sum of the highest $n$ fares in $I$.	
\end{definition}



\begin{definition}
	An online algorithm $P$ (possibly randomized) that incorporates ML-advice is a random function that takes as input an advice $A$, an instance $I = s_1 s_2 \dots s_T$ as history and a fare from $F$; and outputs a binary value (accept/reject decision) that satisfies the capacity constraint, i.e., almost surely it satisfies
	\begin{align*}
		\sum_{t=1}^T P(A, s_1 \dots s_{t-1}, s_t) \leq n	
	\end{align*} 
\end{definition} 

Note that our negative results continue to hold even when the capacity constraint is only required to hold in expectation. Moreover, all our positive results will come from deterministic algorithms.


\begin{definition}
	An online algorithm $P$ is $\beta$-consistent if for any advice $A$, we have
	\begin{align*}
		E\left[\sum_{t=1}^T P(A, s_1 \dots s_{t-1}, s_t) s_t\right] \geq \beta Opt(s_1 \dots s_T)
	\end{align*}
 	where $s_1 \dots s_T$ is the sequence obtained by the following procedure: the first $A_m$ customers are of fare type $f_m$, the next $A_{m-1}$ customers are of fare type $A_{m-1}$, and so on till the last $A_1$ customers who are of fare type $f_1$.  
\end{definition}

\begin{definition}
	An online algorithm $P$ is $\gamma$-competitive if for any advice $A$ and instance $I = s_1 s_2 \dots s_T$, we have
	\begin{align*}
		E\left[\sum_{t=1}^T P(A, s_1 \dots s_{t-1}, s_t) s_t\right] \geq \gamma Opt(s_1 \dots s_T)
	\end{align*}  
\end{definition}

\begin{definition}
	A protection level policy with protection levels $(Q_1, \dots, Q_m)$ is a deterministic online algorithm that, at each time step, accepts as large a fraction of the current customer as possible subject to the condition that the total number of accepted customers of fare $f_i$ or lower never exceeds $Q_i$ for all $i \in [n]$. See page 13 of BQ paper in dropbox folder for a mathematical definition.
\end{definition}




\subsection{ML Advice}

Now, let us consider the setting in which we also have access to an ML oracle that predicts the number of passengers from each fare class that will arrive (this may be restricted to the top $n$ fares). We would like to incorporate this advice in order the improve the performance of our algorithm when the advice is accurate while maintaining the worst-case competitive ratio guarantees of \citet{ball2009toward}. In this section, we will use the notation and terminology introduced  by \citet{lykouris2018competitive} for the study of algorithms with ML advice. We begin by showing that, in the worst-case, no algorithm that is $\beta$-consistent can achieve a competitiveness strictly better than $(1 - \beta)/\Delta$.

\begin{theorem}\label{thm:upper-bound}
	For every algorithm that is $\beta$-consistent and $\gamma$-competitive on all inputs (all possible values of fares $f_1, f_2, \dots, f_m$) with $\beta > 1/ \Delta$, we have $\gamma \leq (1 - \beta)/\Delta$.
\end{theorem}
\begin{proof}
	Set $f_m = 1$ and $f_i = \eta f_{i+1}$ for all $i < m$. Denote with $I_m$ the instance with $n$ consecutive fares of type $f_m$. Next, for $k < m$, define $I_k$ inductively to be the instance $I_{k+1}$ followed by $n$ fares of the type $f_k$.  Assume that the advice is $I_m$. Then any algorithm that is $\beta$-competitive must accept at least $\beta \cdot n$ customers in expectation of type $f_m$ on instance $I_k$ for all $k \in [m]$. If the algorithm is also $\gamma$-competitive, then it must attain at least $\gamma f_k$ revenue on the instance $I_k$ for all $k \in [m]$. As a consequence, it must accept at least $\gamma n - (\beta n f_m/ f_{m-1}) \geq (\gamma - 1/\eta)n$ customers in expectation of the type $f_{m-1}$ in all instances $I_k$ for $k \leq m-1$. By a similar argument, the algorithm needs to accept at least $(\gamma - 1/\eta)n$ customers in expectation of the type $f_k$ in all instances $I_\ell$ for all $\ell \geq k$. But the total number of customers that can be accepted is bounded above by $n$, i.e.,
	\begin{align*}
		\beta n + \sum_{k=1}^{m-1} \left(\gamma - \frac{1}{\eta}\right)n \leq n
	\end{align*}
	Consequently, we get $\gamma \leq \{1 - \beta + (m/\eta)\}/(m-1) \leq [\{1 - \beta + (m/\eta)\}/\Delta] \cdot m/(m-1)$. As $\eta$ and $m$ were arbitrary, setting $\eta = m^2$ and letting $m$ go to infinity completes the proof.
\end{proof}

Next, we describe two simple algorithms, one deterministic and one random, that achieve this upper bound. Fix the consistency parameter $\beta > 1/ \Delta$ such that $\beta n$ is an integer. We will denote the advice by $A = (A_i)_{i=1}^m$. First, we describe the deterministic algorithm. Let $f_k$ be such that there are less than $\beta n$ customers with fare strictly larger than $f_k$ in the advice, call this $q$, and more than $\beta n$ customers with fare greater than or equal to $f_k$. Set $Q'_i = 0$ for $i < k$, $Q'_k = n-q$ and $Q'_i = A_i$ for $i > k$. Furthermore, let $Q_i$ be the protection levels from the policy defined in \citet{ball2009toward} when the capacity is $(1 - \beta)n$. Our deterministic algorithm is simply the protection level algorithm with protection levels $\sum_{j=i}^m Q_j - Q_{j+1} + Q_j' - Q_{j+1}'$ for all $i \in [m]$.

First, note that when the advice is realized, our algorithm accepts at least the top $\beta n$ fares, making it $\beta$-consistent. Next, consider an arbitrary instance $I$. Since the protection levels of our algorithm are all greater than or equal to $Q_i$, it achieves a revenue that is at least $1/\Delta$ fraction of the optimal solution when the capacity is $(1 - \beta)n$. Furthermore, observe that the optimal when the capacity is $(1 - \beta)n$ is at least $(1 - \beta)$ fraction of the optimal when the capacity since the optimal always picks the fares in decreasing order till the capacity if saturated. Combining these observations yields the required $(1 - \beta)/\Delta$ competitiveness. The randomized algorithm can be described as a meta algorithm that takes as input a $\gamma$-competitive algorithm and a $c$-consistent algorithm, and combines them to output a $\beta c$-consistent and $(1 - \beta)\gamma$-competitive algorithm. It does so by simply running the $c$-consistent algorithm with probability $\beta$ and the $\gamma$-competitive algorithm with probability $1 - \beta$.



\subsection{Optimal Protection Level Policy}
 
Protection level policies are central to revenue management both in theory and practice. In the previous section, we gave a simple protection level policy which is optimal in the worst case. But it might be too pessimistic to assume that every aspect of the problem is adversarial. Thus, in this section, we characterize the protection level policy which is optimal for \emph{every} advice. Fix the consistency $\beta$ and competitiveness $\gamma$. Let $A$ be the advice. We will use $Q(I)$ to denote the revenue obtained by the protection level policy determined by protection levels $Q = (Q_1, \dots, Q_m)$ on instance $I$. 

\begin{figure}[h]
\begin{algorithm}[H] 
   \caption{Optimal Protection Level Policy}
   %\textbf{Round}$(\alpha^*,x^*)$
    \begin{algorithmic}\vspace{0.08cm}
            \item[\textbf{For}] $k=m$ to $1$:
            \begin{enumerate}
                \item Set $Q_k$ so to be smallest value that satisfies $Q(I_k) \geq \gamma Opt(I_k)$ and $Q_k \geq Q_{k+1}$
                \item If $Q(A) + \sum_{i=1}^{k-1} A_i f_i < \beta Opt(A)$, increase $Q_k$ so that $Q(A) + \sum_{i=1}^{k-1} A_i f_i = \beta Opt(A)$
            \end{enumerate}
            \item[\textbf{Return:}] $Q$
    \end{algorithmic}
 \end{algorithm}%~\captionof{figure}{The rounding algorithm for $\gamma$-\appe.}\label{fig:alg}
% \medskip\medskip\medskip
\vspace{-4mm}
\end{figure}

First, we use induction to show that step 2 of the for-loop is well-defined. For the base case, note that $Q(A) + \sum_{i=1}^{m-1} A_i f_i \geq \beta Opt(A)$ for $Q_m = A_m$. Hence, step 2 can be executed for $k = m$. Suppose, it can be executed for $k = \ell > 1$. Then, at the end of the $k = \ell$ iteration, we have $Q(A) + \sum_{i=1}^{\ell-1} A_i f_i \geq \beta Opt(A)$. This implies that setting $Q_{\ell-1} = A_{\ell - 1}$ gives $Q(A) + \sum_{i=1}^{\ell-2} A_i f_i \geq \beta Opt(A)$. In other words, step 2 can be executed for $k=\ell-1$, which completes the induction.

The following theorem states that the above algorithm satisfies the capacity constraint if and only if $\beta$-consistency and $\gamma$-consistency are attainable by protection level policies.

\begin{theorem}
	Let $Q$ be the protection levels returned by Algorithm~\ref{alg:opt-protec}. Then, $Q_1 \leq n$ if and only if there exists a protection level algorithm that achieves $\beta$-consistency and $\gamma$-competitiveness.
\end{theorem}
\begin{proof}
	If $Q_1 \leq n$, then to prove the ``only if" direction it suffices to show that the protection level policy with protection levels $Q$ is $\beta$-consistency and $\gamma$-competitive. We get $\gamma$-consistency directly from step 1 of the for-loop, in combination with the results of \citet{ball2009toward} and the fact that the protection levels are only ever increased. On the other hand, we get $\beta$-consistency from the fact that, at the end of the $k=1$ iteration, we have $Q(A) \geq \beta Opt(A)$ by the condition in step 2.
	
	Now, suppose there exists a protection level algorithm ALG with protection levels $Q^*$ that achieves $\beta$-consistency and $\gamma$-competitiveness. Let $Q$ be the protection levels returned by Algorithm~\ref{alg:opt-protec}. We will use induction to show that $Q_k \leq Q^*_k$ for all $k \in [m]$. To do so, we will maintain an auxiliary set of of variables $(x_i)_{i=1}^m$ which we initialize to $x_i = 0$ for all $i \in [m]$ and update them inductively. We will use $x(I)$ to denote the revenue under the protection level policy with $k$-th protection level given by $\sum_{i=k}^m x_i$. 
	
	 For the base iteration $k=m$, first note that we have $Q_m \leq Q_m^*$ after step 1 because ALG attains a revenue of at least $\gamma Opt(I_m)$ on instance $I_m$. On the other hand, since ALG is $\beta$-consistent, we must have $\min\{Q_m^*, A_m\}f_m + \sum_{i=1}^{m-1} A_i f_i \geq \beta Opt(A)$. Therefore, if we set $x_m = Q_m$, then we get $Q(I_m) = x(I_m)$, $Q_m \leq \sum_{i=m}^m x_i$ and $x_m \leq Q^*_m - Q^*_{m+1}$.
	 
	 Suppose, for some $\ell \geq 1$, we have $Q(I_{\ell+1}) = x(I_{\ell+1})$, $Q_{\ell+1} \leq \sum_{i=\ell+1}^m x_i$ and $x_k \leq Q^*_k - Q^*_{k+1}$ for all $k \geq \ell+1$. Update $x$ using the following procedure: for $i=\ell$ to $1$, increase $x_i$ till either $x(I_\ell) = Q(I_\ell)$ or $x_i = Q(i) - Q(i+1)$. Observe that ALG attains a revenue of at least $\gamma Opt(I_\ell)$ on instance $I_\ell$ due to $\gamma$-competitiveness and, if we use $\tilde{A}_k$ to denote the instance obtained by removing fares strictly greater than $f_k$ from $A$, then it also satisfies $Q^*(\tilde{A}_\ell) + \sum_{i=1}^{\ell-1} A_i f_i \geq \beta Opt(A)$ due to $\beta$-consistency. Therefore, the update procedure of $x$ eventually terminates with $x(I_\ell) = Q(I_\ell)$. Also, observe that $Q(I_\ell) = Q(I_{\ell+1}) + (Q_\ell - Q_{\ell+1})f_{\ell}$ and $Q_\ell = Q_{\ell+1} + (Q_\ell - Q_{\ell+1})$. Combining this with the update procedure of $x$, yields $x_\ell \leq Q_\ell - Q_{\ell+1}$. Hence, we have established that $Q(I_{\ell}) = x(I_{\ell})$, $Q_{\ell} \leq \sum_{i=\ell}^m x_i$ and $x_k \leq Q^*_k - Q^*_{k+1}$ for all $k \geq \ell$, which completes the induction.
	 
	 Finally, note that the final step of the induction yields $Q_1 \leq \sum_{i=1}^m x_i \leq \sum_{i=1}^m (Q^*_i - Q^*_{i+1}) = Q^*_1$. Since ALG is a feasible algorithm, it satisfies $Q^*_1 \leq n$, thereby implying $Q_1 \leq n$.
\end{proof}

Next, we give an example where the policy based on Algorithm~\ref{alg:opt-protec} performs better than the worst-case optimal protection level policy described in the previous section.

\par{Example:} Let $f_1 = \eta$, $ f_2 = 1$ and assume $\eta >>1$. Then, $\Delta \approx 0.5$. Moreover, set $n = 10$ and define the instances $I_j$ as in the proof of Theorem~\ref{thm:upper-bound}. Assume that the advice is $I_2$. The worst-case optimal algorithm with $\beta = 0.8$ sets $Q^w_2 \approx 8 + (2/2) = 9$, and $Q^w_1 = 10$ to achieve a competitiveness of $\gamma^w = 0.1$. On the other hand, Algorithm\ref{alg:opt-protec} sets $Q^a_2 = 8$, and $Q^a_1 = 10$ to achieve a competitive ratio of $\gamma^a = 0.2$, which is twice $\gamma^w$.



\subsection{Upper Bound for Randomized Algorithms}

In this section, we will fix the fares $f_1 > f_2 > \dots > f_m$ and establish an upper bound on the best-possible competitiveness for a given level of consistency. Let $\beta > 1/\Delta$ Consider the following LP:
\begin{align*}
	\max \quad &z\\
	 \text{s.t. }& z \leq \frac{\sum_{j=i}^m f_j x_j}{f_i} \quad \forall i \in [m-1] \\
	 & \beta \leq x_m\\
	 &\sum_{i=1}^m x_i \leq 1\\
	 & x_j \geq 0 \quad \forall j \in [m]
\end{align*}

Then, if $(z^*, x^*)$ is the optimal solution to the LP, then the protection level policy with protection levels $Q_i = \sum_{j=i}^m x_j n$ is $\beta$-consistent for the advice $A = I_m$ and $z^*$-competitive. Next, we show that no online policy can achieve a better competitive ratio while maintaining $\beta$-consistency for $I_m$. In other words, no policy can perform strictly better than protection level policies for all advice.

Consider an arbitrary (possibly randomized) online algorithm $P$ which is $\beta$-consistent and $\gamma$-competitive. Let $X_i$ denote the random variable which represents the number of fares of type $f_i$ accepted by $P$ when acting on the instance $I_i$. Note that since $I_i$ is a prefix to $I_j$ for all $1 \leq j \leq i$, $X_i$ is also the number of fares of type $f_i$ accepted when acting on $I_j$ for $j \geq i$. Note that we make no assumption on the correlation structure of the random variables $\{X_i\}$. Set $x_i = E[X_i]/n$ for all $i \in [m]$. Then, the expected revenue of $P$ on $I_i$ is given by $E[\sum_{j=i}^m f_j X_j] = \sum_{j=i}^m f_j x_j n$. Hence, $(\gamma, x)$ is a feasible solution of the LP, and as a consequence $\gamma \leq z^*$.

%The dual is given by
%\begin{align*}
%	\min \quad & r - \beta q \\
%	 \text{s.t. }& r \geq \frac{\sum_{j=1}^i f_i p_j}{f_j} \quad \forall i \in [m-1] \\
%	 & r \geq q + \sum_{j=1}^{m-1} \frac{f_m p_j}{f_j}\\
%	 &\sum_{i=1}^{m-1} p_i = 1\\
%	 & q \geq 0, p_j \geq 0 \quad \forall j \in [m-1]	
%\end{align*}

\subsection{Robustness}

In this subsection, we investigate the degradation in revenue as a function of the proximity of the instance to the advice for Algorithm~\ref{alg:opt-protec}. Consider two advice $A$ and $A'$ which have $k_i$ and $k_i'$ fares of type $f_i$ respectively. Then, we define the distance between them as  $d(A, A') = \sum_{i=1}^m |k_i - k_i'|$. Recall that, where appropriate, we also use $A$ and $A'$ to denote the canonical instances associated with the advice in which the fares arrive in increasing order. In the following, we use $Alg(A, I)$ to represent the performance of Algorithm~\ref{alg:opt-protec} on instance $I$ when it receives advice $A$. Then, $\beta = Alg(A, A)/ Opt(A)$. On advice $A'$ such that $d(A, A') = \ell$ we get
\begin{align*}
	\frac{Alg(A, A)}{Opt(A)} - \frac{Alg(A, A')}{Opt(A')} &= \frac{Alg(A, A)}{Opt(A)} - \frac{Alg(A, A)}{Opt(A')} + \frac{Alg(A, A)}{Opt(A')} - \frac{Alg(A, A')}{Opt(A')}\\
	&= \beta \left\{ \frac{Opt(A') - Opt(A)}{Opt(A')} \right\} + \frac{Alg(A,A) - Alg(A, A')}{Opt(A')}\\
	&\leq \frac{\beta (f_m - f_1)\ell}{f_1 n} + \frac{f_m \ell}{f_1 n}\\
	&\leq \frac{2f_m}{f_1 n} \cdot \ell
\end{align*}

This analysis is almost tight, as demonstrated by the following example.

\paragraph{Example.} 




 


















==> threshold.tex <==
\section{Threshold Policies}

In this section we consider threshold policies, which randomly select a threshold fare before the first customer arrives and only accept fares above that threshold fare. Fix a level of competitiveness $\gamma$ and let $\beta(\gamma)$ be the highest possible consistency achievable by threshold policies that are $\gamma$-competitive. Let $P_\gamma$ be the set of $\gamma$-competitive threshold probabilities, i.e., $x \in P_\gamma$ if and only if 
\begin{align*}
 &\gamma \leq \frac{\sum_{j=i}^m f_j x_j}{f_i} \quad \forall i \in [m] \\
	 &\sum_{i=1}^m x_i \leq 1\\
	 & x_j \geq 0 \quad \forall j \in [m]
\end{align*}

Moreover, let $\mathcal{A}$ be the set of all possible deterministic advice with $\|A\|_1 \geq n \geq \|A\|_\infty$ and $\mathcal{I} = \{I_1, \dots I_m\}$ be the set of advice that consist of increasing fare blocks of size $n$. Consider the following minimax problem (which has value 0):
\begin{align*}
	\min_{D \in \Delta(\mathcal{A})} \max_{x \in P_\gamma} \quad & E_{A \sim D}\left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A)	\right]
\end{align*}

where
\begin{align*}
	c_i(A) = f_i \min\{n, \sum_{\ell=1}^i A_\ell \} + \sum_{j=1}^{i-1} (f_j - f_{j+1}) \left(\min\{n, \sum_{\ell=1}^i A_\ell \} - \sum_{\ell = j + 1}^i A_j\right)^+ 
\end{align*}
and
\begin{align*}
	Opt(A) = f_1 n - \sum_{j=2}^m (f_{j-1} - f_j) \left( n - \sum_{\ell = 1}^{j-1} A_\ell \right)^+
\end{align*}

Then, the following sequence of inequalities hold
\begin{align*}
	\min_{D \in \Delta(\mathcal{I})} \max_{x \in P_\gamma}\ E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right] &\geq \min_{D \in \Delta(\mathcal{A})} \max_{x \in P_\gamma}\ E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right] \\
		&\geq \max_{x \in P_\gamma} \min_{A \in \mathcal{A}}  \sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A)
\end{align*}

Von Neumann minimax theorem implies that
\begin{align*}
	 \max_{x \in P_\gamma} \min_{A \in \mathcal{I}}  \sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) = \min_{D \in \Delta(\mathcal{I})} \max_{x \in P_\gamma}\ E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right]	
\end{align*}

Next, we show that for every fixed threshold probability distribution $x$, there exists a worst case advice in $\mathcal{I}$.

\begin{lemma}\label{lemma:threshold-opt}
	For all $x \in P_\gamma$ and $\alpha \geq 0$, we have $\min_{A \in \mathcal{A}}  \sum_{i=1}^m c_i(A) x_i  - \alpha Opt(A) = \min_{A \in \mathcal{I}}  \sum_{i=1}^m c_i(A) x_i  - \alpha Opt(A)$.
\end{lemma}

\begin{proof}
	Fix an $x \in P_\gamma$. Let $A$ be the advice with the largest $\ell_1$ norm in $\argmin_{A \in \mathcal{A}}  \sum_{i=1}^m c_i(A) x_i  - \alpha Opt(A)$. Suppose $A \notin \mathcal{I}$. We will denote the highest fare in $A$ by $f_h$ and the lowest fare that is a part of $Opt(A)$ as $f_\ell$. Since increasing the number of customers of fare type $f_\ell$ can only decrease $\sum_{i=1}^m c_i(A) x_i  - \alpha Opt(A)$, the maximality of $A$ implies that $A_j = n$ for all $j \geq \ell$. Combining this with the assumption that $A \notin \mathcal{I}$ implies that $A_h < n$. Moreover, as $A$ is maximal, adding a customer of fare type $f_h$ should strictly increase $\sum_{i=1}^m c_i(A) x_i  - \alpha Opt(A)$, i.e.,
	\begin{align*}
		f_h \sum_{j=h}^{\ell-1} x_j > \alpha (f_h - f_\ell)	
	\end{align*}
	But this implies that removing a customer of fare type $f_h$ strictly decreases $\sum_{i=1}^m c_i(A) x_i  - \alpha Opt(A)$, contradicting the definition of $A$.
\end{proof}

Hence, we get that $\max_{x \in P_\gamma} \min_{A \in \mathcal{A}}  \sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) = \max_{x \in P_\gamma} \min_{A \in \mathcal{I}}  \sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A)$. As a consequence, we get
\begin{align*}
	\min_{D \in \Delta(\mathcal{I})} \max_{x \in P_\gamma}\ E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right] = \min_{D \in \Delta(\mathcal{A})} \max_{x \in P_\gamma}\ E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right]	
\end{align*}

Consider the following LP$(D,\gamma)$:
\begin{align*}
	\max \quad & E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right] \\
	 \text{s.t. }& \gamma \leq \frac{\sum_{j=i}^m f_j x_j}{f_i} \quad \forall i \in [m] \\
	 &\sum_{i=1}^m x_i \leq 1\\
	 & x_j \geq 0 \quad \forall j \in [m]
\end{align*}


Now, let us define a new class of policies that take as input a distribution over advice.

\begin{definition}
	An online algorithm $P$ (possibly randomized) that incorporates ML-advice is a random function that takes as input a distribution over instances $D \in \mathcal{A}$ as advice, an instance $I = s_1 s_2 \dots s_T$ as history and a fare from $F$; and outputs a binary value (accept/reject decision) that satisfies the capacity constraint, i.e., almost surely it satisfies
	\begin{align*}
		\sum_{t=1}^T P(D, s_1 \dots s_{t-1}, s_t) \leq n	
	\end{align*} 
\end{definition}

\begin{definition}
	An online algorithm $P$ is $\beta$-consistent if for any advice $D$, we have
	\begin{align*}
		E_{A \sim D}E_P\left[\sum_{t=1}^T P(D, \tilde{A}_{t-1}) s_t\right] \geq \beta E_{A \sim D} \left[Opt(A) \right]
	\end{align*}
	where $\tilde{A}_k$ denotes the instance composed of the $k$ lowest fares in $A$.
\end{definition}

\begin{definition}
	An online algorithm $P$ is $\gamma$-competitive if for any advice $A$ and instance $I = s_1 s_2 \dots s_T$, we have
	\begin{align*}
		E\left[\sum_{t=1}^T P(A, s_1 \dots s_{t-1}, s_t) s_t\right] \geq \gamma Opt(s_1 \dots s_T)
	\end{align*}  
\end{definition}

Consider the following threshold based online algorithm: Solve LP$(D, \gamma)$ described above to obtain the optimal solution $x^*$ and pick a threshold according to $x^*$. We would like to show that this algorithm obtains the optimal consistency level among policies that are $\gamma$-competitive and take as advice a distribution of instances.
 


Let $(D^*, x^*)$ be a saddle point of $\min_{D \in \Delta(\mathcal{I})} \max_{x \in P_\gamma}\ E_{A \sim D} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right]$. Note that, due to the definition of $\beta(\gamma)$, the value of LP$(D^*,\gamma)$ is 0. 

Consider an arbitrary (possibly randomized) online algorithm $P$ that takes a distribution over instances as advice which is $\beta$-consistent and $\gamma$-competitive. Give it advice $D^*$. Let $X_i$ denote the random variable which represents the number of fares of type $f_i$ accepted by $P$ when acting on the instance $I_i$. Note that since $I_i$ is a prefix to $I_j$ for all $1 \leq j \leq i$, $X_i$ is also the number of fares of type $f_i$ accepted when acting on $I_j$ for $j \geq i$. Note that we make no assumption on the correlation structure of the random variables $\{X_i\}$. Set $x_i = E[X_i]/n$ for all $i \in [m]$. Then, the expected revenue of $P$ on $I_i$ is given by $E[\sum_{j=i}^m f_j X_j] = \sum_{j=i}^m f_j x_j n$. Hence, $x$ is a feasible solution of LP$(D^*,\gamma)$ because $P$ is $\gamma$-competitive. Moreover, we can write
\begin{align*}
	 E_{A \sim D^*} \left[\sum_{i=1}^m c_i(A) x_i  - \beta(\gamma) Opt(A) \right]\leq E_{A \sim D^*} \left[\sum_{i=1}^m c_i(A) x^*_i  - \beta(\gamma) Opt(A) \right] = 0 \leq E_{A \sim D^*} \left[\sum_{i=1}^m c_i(A) x_i  - \beta Opt(A) \right]
\end{align*} 

where the first inequality follows from the fact that $x$ is feasible for LP$(D^*, \gamma)$ and $x^*$ is optimal for it, and the last inequality follows from the $\beta$-consistency of $P$ in combination with the fact that $D^*$ is a distribution over $\mathcal{I} = \{I_1, \dots I_m\}$.

Rearranging terms gives $\beta \leq \beta(\gamma)$, proving the optimality of our threshold based policy.


\subsection{In Progress (Deterministic Advice)}

In this section, we will consider fractional advice for the purposes of the proof. For that purpose, set $\mathcal{A}' = \{A \in \R_+ \mid \|A\|_1 \geq n; \|A\|_\infty \leq n\}$. For all $A \in \mathcal{A}'$, define
\begin{align*}
	\hat{c}_i(A) = f_i n + \sum_{j=1}^{i-1} (f_j - f_{j+1}) \left(n - \sum_{\ell = j + 1}^i A_j\right)^+ 
\end{align*}

Observe that $\hat{c}_i(A) \geq c_i(A)$ for all $A \in \mathcal{A}$ and $\hat{c}_i$ is convex. 



Hence, combining this with the concavity of $A \mapsto Opt(A)$ and Lemma~\ref{lemma:threshold-opt} , we can write
\begin{align*}
	\max_{x \in P_\gamma} \min_{A \in \mathcal{I}} \sum_{i=1}^m {c}_i(A) x_i  - \beta(\gamma) Opt(A) &= \max_{x \in P_\gamma} \min_{A \in \mathcal{A}'} \sum_{i=1}^m {c}_i(A) x_i  - \beta(\gamma) Opt(A)\\
	&\leq \min_{A \in \mathcal{A}'} \max_{x \in P_\gamma} \sum_{i=1}^m {c}_i(A) x_i  - \beta(\gamma) Opt(A)\\
	&\leq \min_{A \in \mathcal{A}'} \max_{x \in P_\gamma} \sum_{i=1}^m \hat{c}_i(A) x_i  - \beta(\gamma) Opt(A)\\
	&= \max_{x \in P_\gamma} \min_{A \in \mathcal{A}'} \sum_{i=1}^m \hat{c}_i(A) x_i  - \beta(\gamma) Opt(A)
\end{align*}

where the second to last inequality follows from VN minimax theorem.

Moreover, for all $A \in \mathcal{A}'$ and $i \in [m]$, we have $\hat{c}_i(A) = c(\bar{A})$, where $\bar{A}_1 = n$ and $\bar{A} = A_i$ for all $i \geq 2$.













